Grounding Scene Graphs on Natural Images via Visio-Lingual Message Passing

This paper presents a framework for jointly grounding objects that follow certain semantic relationship constraints given in a scene graph. A typical natural scene contains several objects, often exhibiting visual relationships of varied complexities between them. These inter-object relationships provide strong contextual cues toward improving grounding performance compared to a traditional object query-only-based localization task. A scene graph is an efficient and structured way to represent all the objects and their semantic relationships in the image. In an attempt towards bridging these two modalities representing scenes and utilizing contextual information for improving object localization, we rigorously study the problem of grounding scene graphs on natural images. To this end, we propose a novel graph neural network-based approach referred to as Visio-Lingual Message PAssing Graph Neural Network (VL-MPAG Net). In VL-MPAG Net, we first construct a directed graph with object proposals as nodes and an edge between a pair of nodes representing a plausible relation between them. Then a three-step inter-graph and intra-graph message passing is performed to learn the context-dependent representation of the proposals and query objects. These object representations are used to score the proposals to generate object localization. The proposed method significantly outperforms the baselines on four public datasets.

==> rough.tex <==
% \noindent\textbf{[R1,R2,R4]: Novelity, Message passing explained}:

%\textcolor{red}{do we want to refer that referring expression is a similar problem.}Although a similar area of research, referring expression is more suitable when the query is a short phrase. However, when the goal is to ground a large number of visual entities, i.e., connected via visual relationships between them, on a natural scene, e.g., Fig. 1 in the paper, a short phrase or a sentence would not be sufficient to express all the visual concepts. Instead, a natural language query to perform visual grounding on this scene may look as follows: “A man in a bike and a taxi are moving down a road. Next to the road, there is a woman who is wearing shoes and carrying a bag and an umbrella, walking on a sidewalk. On the orthogonal road, a man holding an umbrella is walking through the zebra crossing. ...”. Using such a lengthy textual description for grounding objects and visual relationships is non-trivial and highly challenging even for modern visual grounding methods due to multiple language understanding challenges that manifolds for long descriptions. Generating such long, complex text queries is not easy especially compared to a corresponding scene graph that can be obtained using a drag-and-drop-based GUI~\cite{Zhang2021GeneAnnotatorAS}.% Further, though attributes are dropped from scene graph for learning attribute-agnostic representations for objects, one can merge nodes corresponding to the object and its attribute into a single node and use it in our framework. Even if we assume that generating natural language queries are easier and more natural to humans, it does not really restrict us from working on scene graph as the query for grounding problem, primarily due to many motivating applications
% that have emerged in recent years. 

% \begin{figure*}[!t]
%     \centering
%     % \captionsetup{type=figure}
%     \includegraphics[width=0.9\textwidth]{figs/goal.png}
% \caption{\label{fig:teasure}\textbf{Our goal: grounding scene graph on image.} Given a scene graph and an image, we aim to localize each object instance represented as individual nodes of the graph along with the semantic relationship between them given by labeled directed edges on the given natural image. \textbf{[Best viewed in color].}}
% \end{figure*}
%-------------------------------------------------------------------------
% In the proposed model, the message passing is performed in three steps. In the first step, the message passing is performed on the auxiliary edges from the query graph to the proposal graph. In this steps, information about the query objects is integrated into the representation of the proposal objects. In the second step, the message passing is performed on the query graph. Representation of the neighboring nodes and edges are used to learn the structured representation of the corresponding nodes. Finally, in the third step, message passing is performed on the constructed proposal graph. This step utilizes the neighborhood information to update the representation of the object proposals. However, if the proposal representations are updated independently of the query nodes, the same proposal representation will be learned for different query scene graphs. This problem is mitigated by the message passing performed in the first step.

% When the order of message-passing in steps one and two are switched, the model observes a drop in performance. This is because the message passing on the auxiliary edges is performed using the updated node representation containing the information about its neighbors leading to less refined messages from the query graph to the proposal graph. We have performed an experiment on the utility of each message passing step and added the results in table 6 on paper.


